Using Nesting to Push the Limits of Transactional Data Structure Libraries

Transactional data structure libraries (TDSL) combine the ease-of-programming of transactions with the high performance and scalability of custom-tailored concurrent data structures. They can be very efficient thanks to their ability to exploit data structure semantics in order to reduce overhead, aborts, and wasted work compared to general-purpose software transactional memory. However, TDSLs were not previously used for complex use-cases involving long transactions and a variety of data structures. In this paper, we boost the performance and usability of a TDSL, towards allowing it to support complex applications. A key idea is nesting. Nested transactions create checkpoints within a longer transaction, so as to limit the scope of abort, without changing the semantics of the original transaction. We build a Java TDSL with built-in support for nested transactions over a number of data structures. We conduct a case study of a complex network intrusion detection system that invests a significant amount of work to process each packet. Our study shows that our library outperforms publicly available STMs twofold without nesting, and by up to 16x when nesting is used.

==> related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Transactional memory.}
Many works have been dedicated to realize atomic transactions
via  \emph{software transactional memory}
approaches~\cite{TL2,Perelman:2011:SSM:2075029.2075041,Herlihy:2003:STM:872035.872048,Perelman:2011:SSM:2075029.2075041}.
Typically, STMs dynamically resolve inconsistencies and
deadlocks by rolling back transactions.
%
However, in spite of a lot of effort, existing STM approaches
have not been widely adopted for real-world concurrent
programming due to various concerns, including high run-time overhead, poor performance and limited applicability~\cite{Cascaval:2008:STM:1454456.1454466}.

In a sense, our transactional skiplist algorithm can be seen as
a combination of the STM TL2
algorithm~\cite{TL2} with techniques for
specialized concurrent data
structures~\cite{fraser2004practical,herlihy-shavit-book}, while
our queues are managed by a different approach that is better
suited for them.
Such optimizations are facilitated by forgoing the generality of
STM toolkits, and restricting transactions to a well-defined set
of data structure operations.


\paragraph{Automatic synchronization via static analysis.}
Several approaches have been proposed to automatically realize
transactions by inferring synchronization via static analysis
algorithms (e.g.,~\cite{CCG:PLDI08,HFP:TRANSACT06,MZGB:POPL06});
some of them deal with high-level data structure
operations~\cite{GGPPOPP:2015}.
In contrast, in this paper we do not rely on static analysis.


%It is interesting to note that, from library's clients
%perspective, our approach can be seen as an \emph{almost
%automatic synchronization approach}, since clients still need to
%correctly handle rollbacks by catching and handling the abort
%exceptions.


\paragraph{Semantic synchronization.}
Some synchronization~ approaches are designed to utilize
semantic properties of data structure operations
(e.g.,~\cite{Herlihy:2008, Koskinen:2010,
KPWRBC:PLDI07, GGPPOPP:2015, Foresight:PLDI13, ni2007open}).
The main idea is to improve parallelism by detecting conflicts
on data structure operations rather than on low level memory
accesses.
In these approaches two commutative data structure operations
can be seen as not conflicting even if their implementations
access the same memory location.
Our approach also employs semantic
synchronization. But in contrast to these previous works, which
only consider the data structure's API, our work also utilizes
the internal structure and implementation details of the data
structure. This allows us to use custom-tailored optimizations such as the
non-transactional index of our skiplist.
Moreover, in contrast to our approach, it is not clear how
semantic approaches can be used to support efficient
singleton operations.


One example of a semantic approach is boosting \cite{Herlihy:2008}, which
presents a methodology for bundling linearizable object operations into transactions.
Boosting is based on a semantic variant of two phase locking,
in which the data structure operations are protected by a set of abstract locks.
Boosting has a number of limitations, including restricted generality (for example, it is not clear how to efficiently implement a thread-safe iterator), the need to support compensating actions via bookkeeping, and sensitivity to
parameters (like the timeouts which are used to detect deadlocks).

Another example of semantic synchronization is open nesting~\cite{ni2007open}.
However, this approach 
%while users of our library are only required to wrap up
%the operations they wish to perform, inside a transaction,
%between \emph{TX-begin} and \emph{TX-commit}, the implementation of open
%nested transactions in~\cite{ni2007open} 
is intended for experienced programmers, as it requires programmers to explicitly
use abstract locks and also to provide an abstract compensating action for each of its open nested
transactions, to be used in case of abort.
%In addition, it is not clear how open nesting can be used to support fast singleton operations.

Our approach is inspired by the idea
of foresight~\cite{Foresight:PLDI13}, which also supports atomicity of a number of CDSL operations.
But in contrast to our library, it requires external information
about the transactions' code, which is computed via static
analysis.
%
Furthermore, our solution utilizes optimistic synchronization
(transactions may be aborted), whereas synchronization in foresight
\cite{Foresight:PLDI13} is fully pessimistic (transactions are
never aborted).


\paragraph{Composing operations.}
Several works have suggested approaches for composing multiple
CDSL operations into larger atomic operations.
One example is reagents~\cite{turon2012reagents}, 
which provides a set of building blocks for
writing concurrent data structures and synchronizers that express concurrency algorithms at a higher
level of abstraction.
However, with reagents, concurrency control is not transparent
to the programmer. 
In particular, reagents programmers need to use non-trivial
fine-grained data structure operations and put them together in
a way that implements the desired functionality.

Another recent example is RLU~\cite{matveev2015read}, which is
a tool to compose multiple data structure updates in a way that
does not hamper the efficiency of data structure read-only
operations.
Similarly to our work, their work is also inspired by STM mechanisms for 
synchronizing between readers and writers that wish to update
multiple locations atomically. But in contrast to us, they provide a
tool for building efficient complex CDSLs (e.g., doubly
linked lists) rather than TDSLs.


%A recent approach~\cite{turon2012reagents}, called reagents,
%proposed a way to compose sequence of operations together to
%provide atomic move operations between different collection data
%types.
%They provide a set of building blocks for
%writing concurrent data structures and synchronizers that allow
%them to express concurrency algorithms at a higher
%level of abstraction.
%However, with reagents, concurrency control is not transparent
% to the programmer. In particular, reagents programmers
%need to use non-trivial fine-grained data structure operations
% and put them together in a way that implements the desired functionality.




\paragraph{Data structures for STMs.}
Some works describe data structures that are compatible with
STMs~\cite{Marathe:2007,
Bronson:PODC:2010,crain2012contention,STO-euorosys2016}.
Similarly to our skiplist, they use operation semantics to
reduce the read-set size, leading to fewer aborts and smaller
validation overhead. 
The data structures in
\cite{Marathe:2007,STO-euorosys2016} and
\cite{Bronson:PODC:2010} translate their high-level operations
into low level ones, and the transaction-friendly
skiplist~\cite{crain2012contention} delays some non-critical
work that may lead to aborts to a dedicated thread that runs in
the background. These data structures are designed to correctly
and efficiently work within STM transactions, and do not include
support for fast abort-free singletons as we provide.
Furthermore, whereas in our approach the synchronization
algorithm is part of the library implementation, in these works,
the actual synchronization algorithm (or at least part of it) is
implemented outside the data structure library, i.e., handled by
the external STM. Therefore, their data structures must expose
some abstract conflict information for the STM to use. This may
limit data structure implementations, for example, our
non-transactional index, our fast singletons, (which do not
update the GVC), and the ordered write-set we use in the queue
are not readily amenable to such abstract representations.
\emph{Software transactional objects}
(STO)~\cite{STO-euorosys2016}, which were developed
independently and concurrently with our work, advocate co-design
of the transactional data structures and the STM.

